Insider Stories: Analyzing Internal Sustainability Efforts of Major US Companies from Online Reviews

It is hard to establish whether a company supports internal sustainability efforts (ISEs) like gender equality, diversity, and general staff welfare, not least because of lack of methodologies operationalizing these internal sustainability practices, and of data honestly documenting such efforts. We developed and validated a six-dimension framework reflecting Internal Sustainability Efforts (ISEs), gathered more than 350K employee reviews of 104 major companies across the whole US for the (2008-2020) years, and developed a deep-learning framework scoring these reviews in terms of the six ISEs. Commitment to ISEs manifested itself at micro-level -- companies scoring high in ISEs enjoyed high stock growth. This new conceptualization of ISEs offers both theoretical implications for the literature in corporate sustainability, and practical implications for companies and policymakers. To further explore these implications, researchers need to add potentially missing ISEs, to do so for more companies, and establish the causal relationship between company success and ISEs.

==> old_tex_files/old_intro.tex <==
Investments in sustainability are becoming paramount as many companies are under constant pressure to reduce the social and environmental impact of their operations~\cite{bai2020supply} and increase accountability towards stakeholders and the wider society ~\cite{de2021reimaginingmol2015transparency,serafeim2020social}. While corporate sustainability efforts tend to focus primarily on external stakeholders (e.g., customers, supply-chain partners, governmental organizations)~\cite{doi:10.1177/0022242921992052}, internal stakeholders (e.g., employees) represent a critical, and sometimes overlooked, target group to ensure effective corporate engagement with the sustainability agenda~\cite{martin2021exploring,paine2014sustainability}. 

Internal sustainability efforts (ISEs) encompass a wide range of corporate policies directed towards internal stakeholders, including, for example, promoting a healthy employee work-life balance~\cite{kelliher2019all}, investing in gender equality and diversity~\cite{NADEEM2017874}, or ensuring an harassment-free working environment~\cite{cassino2019race}. These ISEs can reduce staff turnover~\cite{giauque2019stress} and improve market competitiveness~\cite{wang2012explaining}. However, although many companies openly advertise their commitment to internal sustainability, employees often report contrasting accounts of their experience of such efforts~\cite{peloza2011how}, and the extent to which ISEs successfully propagate throughout the organization remains unclear. Reflecting on these critical issues, this paper presents a large-scale assessment of organizational practices aligned with ISEs and empirically interrogates how these internal efforts influence a company's market performance.

Since there exists no agreed-upon definition of corporate's ISEs, to inform our research we start from the United Nations (UN) World Commission on Environment and Development (WCED) definition of sustainability as a strategy oriented towards “meeting the needs of the present without compromising the ability of future generations to meet their own needs”~\cite{wced1987world}. This definition is operationalized in the UN 17 sustainable development goals (SDGs) that represent both a framework and a call-to-action for organizations to invest in addressing critical societal issues such as “good health and well-being,” “decent work and economic growth,” and “peace, justice and strong institutions”~\cite{nations2015transforming}. Taken together, the SDGs highlight the most important strategic imperatives that companies and other organizations should consider when investing in sustainability~\cite{giannetti2020cleaner,govindan2020achieving}. Not all 17 UN SDGs are however relevant to a company's {\em internal} stakeholders; this is the case, for example, of goals such as `life under water'. To identify those that are relevant to a company's employees, and to sharpen their definition in such context, we use the UN SDGs as starting point to then examine more than 350K geo-referenced reviews about S\&P 500 companies, published by current and former employees on a popular company reviewing website between 2008 and 2020. We then develop and validate a mixed-method approach that paraphrases the broad UN SDGs into corporate-relevant internal sustainability efforts. Core to the approach is a state-of-the-art Natural Language Processing (NLP) framework to delineate companies ISEs from employees’ reviews, together with robust measures of corporate engagement with these ISEs. Next, we employ the validated measures to assess how ISEs influence a company financial standing, and examine how companies in different sectors perform on our validated ISEs measures. Lastly, we assess how corporate engagement with internal sustainability manifests itself at a macroeconomic and societal level.

Our research offers three substantive contributions to the multidisciplinary research on sustainability. First, we develop and empirically validate a NLP framework that accurately delineates the micro foundations of sustainability efforts from the perspective of a company's employees. Our framework allows future researchers and managers to quantify and qualify the extent to which corporate engagement with ISEs becomes visible to employees across different organizational levels. Second, we identify two core dimensions of ISEs, namely \textit{financial sustainability efforts} (e.g., employee financial compensation and financial benefits) and \textit{welfare sustainability efforts} (e.g., investments in gender equality policies) (Figure~\ref{fig:wheel}). These dimensions represent the main areas of strategic focus for companies oriented towards internal sustainability. Third, we show that corporate engagement with ISEs leads to market performance improvement. In particular, we find that companies with high level of engagement with ISEs enjoy higher financial growth, and that the IT and industrial goods sectors are currently leading on ISEs engagement. Furthermore, we show that the benefits of ISEs engagement reap at macroeconomic level. In particular, a state-level analysis reveals that US states that host companies engaging with ISEs reach higher levels of wealth, economic equality, and creativity. Policymakers should consider schemes that encourage corporate sponsorship of, and investments in, ISEs to stimulate states' socioeconomic development. 

==> old_tex_files/old_state_regressions.tex <==
\subsection*{Does sustainability have consequences for state outcomes?} 

We now turn to how sustainability perceptions affects state level indicators. 

\textbf{Predicting wealth, income inequality, and creativity from ISEs.}  
%\todo{in this section, add correlations with emerging}
The previous results suggest that states with companies that value sustainability practices tend to be wealthy, economically equal, and creative. Indeed, a state's wealth (GDP per capita) is positively correlated with the composite sustainability score $[r=0.37, P=0.008]$ 
(Figure~\ref{fig:gdp_gini_cc_regressions}) and its strongest correlation is with  sustainability practices around a ``supportive environment'' $[r=0.48, P=0.000]$, -which suggests that fostering a supportive work environment, through positive management or helpful co-workers, was associated with greater state wealth. 

By contrast, a state's income inequality (Gini Coefficient) is negatively correlated with the composite sustainability score $[r=-0.29, P=0.043]$ (Figure \ref{fig:gdp_gini_cc_regressions}), and its strongest (negative) correlation is with  sustainability practices around ``financial benefits'' $[r=-0.54, P=0.008]$, which suggests that more equal states enjoy greater employee satisfaction with respect to decent wages and economic benefits.

Finally, a state's creativity  is positively correlated with the composite sustainability score $[r=0.31, P=0.030]$ (Figure \ref{fig:gdp_gini_cc_regressions}), and its strongest  correlation is with  sustainability practices around ``work environment''  $[r=0.51, P=0.000]$, which suggest that creativity and infrastructure availability are strongly associated, as is the presence of creative professional in IT areas who express ISEs connected to infrastructure.


\begin{table}[t] \centering \scriptsize
\begin{tabular}{@{\extracolsep{5pt}}lcccccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
\\[-1.8ex] & wealth (composite) & wealth (best) & inequality (composite) & inequality (best) & creativity (composite) & creativity (best) \\
\hline \\[-1.8ex]
const & 11.875$^{}$ & 9.681$^{}$ & 40.365$^{***}$ & 48.337$^{***}$ & 25.366$^{***}$ & 18.872$^{**}$ \\
  & (9.882) & (9.377) & (9.665) & (8.943) & (8.648) & (7.572) \\
 urban population & 0.440$^{***}$ & 0.406$^{***}$ & 0.284$^{**}$ & 0.182$^{}$ & 0.532$^{***}$ & 0.458$^{***}$ \\
  & (0.129) & (0.124) & (0.126) & (0.109) & (0.113) & (0.100) \\
 financial benefits & & & & -0.558$^{***}$ & & \\
  & & & & (0.124) & & \\
 financial\_vs\_emerging score & & 0.344$^{***}$ & & & & 0.370$^{***}$ \\
  & & (0.118) & & & & (0.096) \\
 composite score & 0.318$^{**}$ & & -0.416$^{***}$ & & 0.177$^{}$ & \\
  & (0.157) & & (0.154) & & (0.138) & \\
\hline \\[-1.8ex]
 Observations & 50 & 50 & 50 & 50 & 50 & 50 \\
 $R^2$ & 0.310 & 0.364 & 0.172 & 0.332 & 0.385 & 0.517 \\
 Adjusted $R^2$ & \textbf{0.281} & \textbf{0.337} & \textbf{0.137} & \textbf{0.304} & \textbf{0.359} & \textbf{0.497} \\
 Residual Std. Error & 20.972(df = 47) & 20.131(df = 47) & 20.510(df = 47) & 18.419(df = 47) & 18.352(df = 47) & 16.257(df = 47)  \\
 F Statistic & 10.561$^{***}$ & 13.466$^{***}$ & 4.884$^{**}$ & 11.696$^{***}$ & 14.721$^{***}$ & 25.204$^{***}$ \\
 & (df = 2.0; 47.0) & (df = 2.0; 47.0) & (df = 2.0; 47.0) & (df = 2.0; 47.0) & (df = 2.0; 47.0) & (df = 2.0; 47.0) \\
\hline
\hline \\[-1.8ex]
\textit{Note:} & \multicolumn{6}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}
\caption{OLS models predicting state wealth (GDP per capita), inequality (Gini coefficient), and creativity index (logged) from a stepAIC analysis. All variables are scaled between 0 and 100 to aid in interpretability.}
\label{tab:gdp_gini_cc}
\end{table}


A considerable body of literature has shown that those three socio-economic conditions are associated with the agglomeration of the creative class in urban areas~\cite{florida2005cities,bonaventura2021predicting}\todo{which reference is `PNAS'?}. To test that, we predicted the three socio-economic conditions  from a state's composite sustainability score $S(u)$ while controlling for urbanization.  The combination of urbanization and the composite sustainability score alone explained 28\% of the variability in wealth, 14\% of inequality, and 36\% of creativity (Table~\ref{tab:gdp_gini_cc}). Then, by replacing the composite score with the strongest correlated type of sustainability practices 
%(the three variables at the bottom panel of Figure~\ref{fig:sanity_regressions}) 
and combining it with urbanization, we explained 32\% of the variability in wealth, 30\% of inequality, and 48\% of creativity. In comparison, only urbanization explains 24\%, 2\%, and 35\% variability in wealth, inequality, and creativity, respectively. 

Essentially, we found that wealth co-occurs with urban areas that tend to offer employers who values the creation of supportive environment and management. On the other hand, more equal states tend to have employees who focus on practices around financial benefits. Finally, creative states tend to have employees who value access to infrastructure and technology.

The emerging sustainability score is much more strongly correlated with wealth $[r = , p < 0.001]$ and creativity $[r = , p < 0.001]$, implying that wealthier and more creative states invest in more non-traditional types of sustainability. 


==> old_tex_files/sustainability_pred_tables.tex <==
% without interaction

\begin{table}[!htbp] 
\centering
\scriptsize
\begin{tabular}{@{\extracolsep{5pt}}lccccccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
\\[-1.8ex] & composite & health & education & gender & finance & infrastructure & supportive \\
\hline \\[-1.8ex]
 const & -2.167$^{}$ & 17.421$^{*}$ & 42.681$^{***}$ & 23.665$^{**}$ & 54.279$^{***}$ & 11.565$^{}$ & -3.021$^{}$ \\
  & (2.078) & (9.286) & (7.964) & (8.978) & (5.662) & (8.811) & (13.439) \\
 creativity & & 0.292$^{**}$ & & & & 0.387$^{**}$ & 0.347$^{***}$ \\
  & & (0.142) & & & & (0.148) & (0.124) \\
 cultural
tightness & & & & & & & 0.200$^{}$ \\
  & & & & & & & (0.122) \\
 inequality & -0.105$^{***}$ & -0.341$^{***}$ & -0.217$^{*}$ & -0.347$^{**}$ & -0.522$^{***}$ & & -0.294$^{**}$ \\
  & (0.035) & (0.120) & (0.114) & (0.151) & (0.117) & & (0.113) \\
 lgbtq
travel & & & & & & 0.397$^{***}$ & \\
  & & & & & & (0.146) & \\
 total
reviews & 0.065$^{**}$ & & & 0.262$^{*}$ & & & \\
  & (0.032) & & & (0.137) & & & \\
 urbanization & & 0.220$^{}$ & & & & -0.237$^{*}$ & \\
  & & (0.133) & & & & (0.140) & \\
 wealth & 0.062$^{**}$ & & 0.282$^{***}$ & 0.280$^{**}$ & & & 0.325$^{***}$ \\
  & (0.027) & & (0.102) & (0.118) & & & (0.109) \\
\hline \\[-1.8ex]
 Observations & 50 & 50 & 50 & 50 & 50 & 50 & 50 \\
 $R^2$ & 0.282 & 0.302 & 0.196 & 0.247 & 0.293 & 0.367 & 0.374 \\
 Adjusted $R^2$ & 0.235 & 0.257 & 0.162 & 0.198 & 0.278 & 0.326 & 0.319 \\
 Residual Std. Error & 4.548(df = 46) & 17.943(df = 46) & 17.649(df = 47) & 19.652(df = 46) & 18.078(df = 48) & 17.583(df = 46) & 15.810(df = 45)  \\
 F Statistic & 6.031$^{***}$ & 6.646$^{***}$ & 5.726$^{***}$ & 5.027$^{***}$ & 19.872$^{***}$ & 8.899$^{***}$ & 6.732$^{***}$ \\
 & (df = 3.0; 46.0) & (df = 3.0; 46.0) & (df = 2.0; 47.0) & (df = 3.0; 46.0) & (df = 1.0; 48.0) & (df = 3.0; 46.0) & (df = 4.0; 45.0) \\
\hline
\hline \\[-1.8ex]
\textit{Note:} & \multicolumn{7}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}
\caption{Predicting sustainability with state-level socio-economic indicators (without interactions)}
\label{6goals_no_interactions}
\end{table}

\begin{comment}

% without negative interaction
\begin{table}[!htbp] \centering
\scriptsize
\begin{tabular}{@{\extracolsep{5pt}}lccccccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
\\[-1.8ex] & composite & health & education & gender & finance & infrastructure & supportive \\
\hline \\[-1.8ex]
 const & -6.955$^{**}$ & 30.933$^{***}$ & 22.372$^{**}$ & 20.590$^{**}$ & 149.950$^{***}$ & 48.058$^{**}$ & 10.911$^{}$ \\
  & (2.769) & (7.691) & (10.931) & (9.631) & (43.078) & (20.660) & (9.337) \\
 creativity & 0.073$^{*}$ & & 0.228$^{}$ & & & 0.462$^{***}$ & 0.299$^{**}$ \\
  & (0.036) & & (0.151) & & & (0.154) & (0.133) \\
 cultural
tightness & & & & & -1.940$^{**}$ & & \\
  & & & & & (0.821) & & \\
 cultural tightness *
wealth & 0.067$^{**}$ & 0.187$^{}$ & 1.259$^{**}$ & & 2.058$^{**}$ & 0.300$^{*}$ & 0.234$^{**}$ \\
  & (0.030) & (0.121) & (0.553) & & (0.811) & (0.153) & (0.111) \\
 inequality & -0.100$^{***}$ & -0.428$^{***}$ & -0.335$^{***}$ & -0.319$^{**}$ & -0.563$^{***}$ & -0.352$^{**}$ & -0.337$^{***}$ \\
  & (0.031) & (0.126) & (0.122) & (0.130) & (0.132) & (0.150) & (0.107) \\
 lgbtq
travel & 0.051$^{}$ & & 1.077$^{**}$ & & & 0.379$^{**}$ & \\
  & (0.035) & & (0.500) & & & (0.150) & \\
 lgbtq travel*
creativity & & & & & -0.282$^{*}$ & & \\
  & & & & & (0.160) & & \\
 lgbtq travel*
cultural tightness & & & -1.314$^{*}$ & 0.291$^{*}$ & & & \\
  & & & (0.665) & (0.152) & & & \\
 urbanization & & & & & & -1.001$^{***}$ & \\
  & & & & & & (0.371) & \\
 urbanization*
creativity & & 0.414$^{***}$ & & & & & \\
  & & (0.100) & & & & & \\
 urbanization*
wealth & & & & 0.347$^{***}$ & 0.542$^{**}$ & 1.443$^{**}$ & 0.214$^{*}$ \\
  & & & & (0.112) & (0.265) & (0.658) & (0.117) \\
 wealth & & & -0.595$^{}$ & & -1.690$^{**}$ & -0.931$^{**}$ & \\
  & & & (0.381) & & (0.676) & (0.451) & \\
\hline \\[-1.8ex]
 Observations & 50 & 50 & 50 & 50 & 50 & 50 & 50 \\
 $R^2$ & 0.334 & 0.317 & 0.323 & 0.261 & 0.438 & 0.463 & 0.392 \\
 Adjusted $R^2$ & 0.275 & 0.272 & 0.229 & 0.213 & 0.360 & 0.374 & 0.338 \\
 Residual Std. Error & 4.430(df = 45) & 17.759(df = 46) & 16.928(df = 43) & 19.467(df = 46) & 17.024(df = 43) & 16.947(df = 42) & 15.590(df = 45)  \\
 F Statistic & 5.640$^{***}$ & 7.105$^{***}$ & 3.423$^{***}$ & 5.417$^{***}$ & 5.590$^{***}$ & 5.180$^{***}$ & 7.243$^{***}$ \\
 & (df = 4.0; 45.0) & (df = 3.0; 46.0) & (df = 6.0; 43.0) & (df = 3.0; 46.0) & (df = 6.0; 43.0) & (df = 7.0; 42.0) & (df = 4.0; 45.0) \\
\hline
\hline \\[-1.8ex]
\textit{Note:} & \multicolumn{7}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}
\caption{Predicting sustainability with state-level socio-economic indicators (without negative interactions)}
\label{tab:6goals_minus_neg_interactions}
\end{table}

% with all interactions
\begin{table}[!htbp] \centering
\scriptsize
\begin{tabular}{@{\extracolsep{5pt}}lccccccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
\\[-1.8ex] & composite & health & education & gender & finance & infrastructure & supportive \\
\hline \\[-1.8ex]
 const & 23.906$^{**}$ & 112.893$^{**}$ & 1.003$^{}$ & -1.765$^{}$ & 149.950$^{***}$ & 119.246$^{***}$ & 117.062$^{***}$ \\
  & (11.370) & (45.057) & (20.974) & (13.844) & (43.078) & (42.607) & (39.869) \\
 cultural
tightness & -0.619$^{***}$ & -2.043$^{**}$ & & & -1.940$^{**}$ & -2.093$^{**}$ & -2.216$^{***}$ \\
  & (0.217) & (0.866) & & & (0.821) & (0.796) & (0.766) \\
 cultural tightness *
wealth & 0.673$^{***}$ & 2.274$^{**}$ & & 0.242$^{*}$ & 2.058$^{**}$ & 2.171$^{***}$ & 2.436$^{***}$ \\
  & (0.216) & (0.859) & & (0.143) & (0.811) & (0.790) & (0.761) \\
 inequality & -0.143$^{***}$ & -0.589$^{***}$ & -0.185$^{}$ & -0.351$^{**}$ & -0.563$^{***}$ & -0.446$^{***}$ & -0.456$^{***}$ \\
  & (0.035) & (0.139) & (0.117) & (0.144) & (0.132) & (0.130) & (0.123) \\
 lgbtq
travel & 0.431$^{***}$ & 1.724$^{***}$ & 0.981$^{***}$ & 1.345$^{***}$ & & 2.185$^{***}$ & 1.346$^{***}$ \\
  & (0.114) & (0.452) & (0.361) & (0.499) & & (0.414) & (0.400) \\
 lgbtq travel*
creativity & 0.085$^{}$ & & & & -0.282$^{*}$ & 1.398$^{**}$ & \\
  & (0.052) & & & & (0.160) & (0.569) & \\
 lgbtq travel*
urbanization & -0.784$^{***}$ & -3.016$^{***}$ & -1.294$^{**}$ & -1.704$^{**}$ & & -4.056$^{***}$ & -2.599$^{***}$ \\
  & (0.187) & (0.745) & (0.517) & (0.753) & & (0.726) & (0.659) \\
 total reviews*
lgbtq travel & 2.043$^{***}$ & 8.799$^{***}$ & & & & 5.391$^{**}$ & 9.236$^{***}$ \\
  & (0.653) & (2.702) & & & & (1.993) & (2.391) \\
 total reviews*
urbanization & -0.609$^{}$ & -3.113$^{*}$ & & & & & -3.249$^{**}$ \\
  & (0.444) & (1.802) & & & & & (1.595) \\
 total reviews*creativity & -1.399$^{**}$ & -5.469$^{**}$ & & & & -5.235$^{**}$ & -5.843$^{***}$ \\
  & (0.547) & (2.159) & & & & (1.975) & (1.910) \\
 urbanization & & & 0.410$^{}$ & & & & \\
  & & & (0.293) & & & & \\
 urbanization*
creativity & & 0.420$^{**}$ & & & & -0.793$^{}$ & 0.411$^{**}$ \\
  & & (0.204) & & & & (0.549) & (0.180) \\
 urbanization*
wealth & 0.903$^{***}$ & 3.454$^{***}$ & 0.466$^{**}$ & 1.825$^{**}$ & 0.542$^{**}$ & 4.444$^{***}$ & 2.936$^{***}$ \\
  & (0.203) & (0.826) & (0.195) & (0.780) & (0.265) & (0.935) & (0.731) \\
 wealth & -0.944$^{***}$ & -3.527$^{***}$ & & -0.934$^{*}$ & -1.690$^{**}$ & -4.048$^{***}$ & -3.131$^{***}$ \\
  & (0.224) & (0.887) & & (0.488) & (0.676) & (0.896) & (0.785) \\
\hline \\[-1.8ex]
 Observations & 50 & 50 & 50 & 50 & 50 & 50 & 50 \\
 $R^2$ & 0.570 & 0.572 & 0.302 & 0.359 & 0.438 & 0.661 & 0.605 \\
 Adjusted $R^2$ & 0.445 & 0.449 & 0.222 & 0.269 & 0.360 & 0.562 & 0.490 \\
 Residual Std. Error & 3.874(df = 38) & 15.457(df = 38) & 16.999(df = 44) & 18.754(df = 43) & 17.024(df = 43) & 14.167(df = 38) & 13.677(df = 38)  \\
 F Statistic & 4.578$^{***}$ & 4.624$^{***}$ & 3.801$^{***}$ & 4.012$^{***}$ & 5.590$^{***}$ & 6.726$^{***}$ & 5.284$^{***}$ \\
  & (df = 11.0; 38.0) & (df = 11.0; 38.0) & (df = 5.0; 44.0) & (df = 6.0; 43.0) & (df = 6.0; 43.0) & (df = 11.0; 38.0) & (df = 11.0; 38.0) \\
\hline
\hline \\[-1.8ex]
\textit{Note:} & \multicolumn{7}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}
\caption{Predicting sustainability with state-level socio-economic indicators with all interactions between variables that have at least $|0.5|$ correlation}
\label{tab:6goals}
\end{table}


\begin{table}[!htbp] \centering
\scriptsize
\begin{tabular}{@{\extracolsep{5pt}}lccccccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
\\[-1.8ex] & composite & health & education & gender & finance & infrastructure & supportive \\
 const & -2.167$^{}$ & -16.050$^{}$ & 42.681$^{***}$ & 23.665$^{**}$ & 54.279$^{***}$ & 32.054$^{**}$ & -3.021$^{}$ \\
  & (2.078) & (21.417) & (7.964) & (8.978) & (5.662) & (15.049) & (13.439) \\
 creativity & & & & & & & 0.347$^{***}$ \\
  & & & & & & & (0.124) \\
 cultural
tightness & & & & & & & 0.200$^{}$ \\
  & & & & & & & (0.122) \\
 freedom & & & & & & -0.253$^{*}$ & \\
  & & & & & & (0.142) & \\
 inequality & -0.105$^{***}$ & -0.309$^{**}$ & -0.217$^{*}$ & -0.347$^{**}$ & -0.522$^{***}$ & -0.315$^{**}$ & -0.294$^{**}$ \\
  & (0.035) & (0.126) & (0.114) & (0.151) & (0.117) & (0.144) & (0.113) \\
 lgbtq
travel & & 0.779$^{**}$ & & & & 0.806$^{***}$ & \\
  & & (0.361) & & & & (0.241) & \\
 lgbtq travel*
creativity & & 0.404$^{**}$ & & & & & \\
  & & (0.197) & & & & & \\
 lgbtq travel*
urbanization & & -1.285$^{**}$ & & & & -0.900$^{***}$ & \\
  & & (0.553) & & & & (0.279) & \\
 total
reviews & 0.065$^{**}$ & & & 0.262$^{*}$ & & 0.240$^{}$ & \\
  & (0.032) & & & (0.137) & & (0.170) & \\
 urbanization & & 0.848$^{***}$ & & & & & \\
  & & (0.308) & & & & & \\
 urbanization*
creativity & & & & & & 0.504$^{***}$ & \\
  & & & & & & (0.181) & \\
 wealth & 0.062$^{**}$ & & 0.282$^{***}$ & 0.280$^{**}$ & & & 0.325$^{***}$ \\
  & (0.027) & & (0.102) & (0.118) & & & (0.109) \\
\hline \\[-1.8ex]
 Observations & 50 & 50 & 50 & 50 & 50 & 50 & 50 \\
 $R^2$ & 0.282 & 0.370 & 0.196 & 0.247 & 0.293 & 0.479 & 0.374 \\
 Adjusted $R^2$ & 0.235 & 0.299 & 0.162 & 0.198 & 0.278 & 0.406 & 0.319 \\
 Residual Std. Error & 4.548(df = 46) & 17.433(df = 44) & 17.649(df = 47) & 19.652(df = 46) & 18.078(df = 48) & 16.502(df = 43) & 15.810(df = 45)  \\
 F Statistic & 6.031$^{***}$  & 5.171$^{***}$  & 5.726$^{***}$ & 5.027$^{***}$ & 19.872$^{***}$ & 6.590$^{***}$ & 6.732$^{***}$ \\
 & (df = 3.0; 46.0) & (df = 5.0; 44.0) & (df = 2.0; 47.0) & (df = 3.0; 46.0) & (df = 1.0; 48.0) & (df = 6.0; 43.0) & (df = 4.0; 45.0) \\
\hline
\hline \\[-1.8ex]
\textit{Note:} & \multicolumn{7}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}
\caption{Predicting sustainability with state-level socio-economic indicators with all interactions between variables that have at least $|0.6|$ correlation}
\label{tab:6goals_atleast_60}
\end{table}

\end{comment}

==> old_tex_files/tables.tex <==
% \begin{table}[!htbp] \centering \scriptsize
% \begin{tabular}{@{\extracolsep{5pt}}lcccccc}
% \\[-1.8ex]\hline
% \hline \\[-1.8ex]
% \\[-1.8ex] & wealth (composite) & wealth (best) & inequality (composite) & inequality (best) & creativity (composite) & creativity (best) \\
% \hline \\[-1.8ex]
% const & 11.875$^{}$ & 12.566$^{}$ & 40.365$^{***}$ & 48.337$^{***}$ & 25.366$^{***}$ & 16.385$^{**}$ \\
%   & (9.882) & (9.231) & (9.665) & (8.943) & (8.648) & (8.001) \\
%  EV: supportive environment & & 0.434$^{**}$ & & & & \\
%   & & (0.164) & & & & \\
%  EV: pay, economic & & & & -0.558$^{***}$ & & \\
%   & & & & (0.124) & & \\
%  EV: work environment & & & & & & 0.415$^{***}$ \\
%   & & & & & & (0.113) \\
%   sustainability score scaled & 0.318$^{**}$ & & -0.416$^{***}$ & & 0.177$^{}$ & \\
%   & (0.157) & & (0.154) & & (0.138) & \\
%  urbanPop & 0.440$^{***}$ & 0.383$^{***}$ & 0.284$^{**}$ & 0.182$^{}$ & 0.532$^{***}$ & 0.484$^{***}$ \\
%   & (0.129) & (0.130) & (0.126) & (0.109) & (0.113) & (0.100) \\
% \hline \\[-1.8ex]
%  Observations & 50 & 50 & 50 & 50 & 50 & 50 \\
%  $R^2$ & 0.310 & 0.348 & 0.172 & 0.332 & 0.385 & 0.505 \\
%  Adjusted $R^2$ & 0.281 & 0.320 & 0.137 & 0.304 & 0.359 & 0.484 \\
%  Residual Std. Error & 20.972(df = 47) & 20.391(df = 47) & 20.510(df = 47) & 18.419(df = 47) & 18.352(df = 47) & 16.464(df = 47)  \\
%  F Statistic & 10.561$^{***}$ & 12.528$^{***}$ & 4.884$^{**}$ & 11.696$^{***}$ & 14.721$^{***}$  & 23.989$^{***}$  \\
%   & (df = 2.0; 47.0) & (df = 2.0; 47.0) & (df = 2.0; 47.0) & (df = 2.0; 47.0) & (df = 2.0; 47.0) &  (df = 2.0; 47.0) \\
% \hline
% \hline \\[-1.8ex]
% \textit{Note:} & \multicolumn{6}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
% \end{tabular}
% \caption{OLS models predicting state GDP, Gini coefficient, and creativity index (logged). Running stepAIC reveals that the full model is the minimal model in both cases. All variables are scaled between 0 and 100 to aid in interpretability.}
% \label{tab:gdp_gini_cc}
% \end{table}


\begin{comment}

\begin{table}[!htbp] \centering \scriptsize
\begin{tabular}{@{\extracolsep{5pt}}lcccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
\\[-1.8ex] & Wealth (composite) & wealth (best facet) & inequality (composite) & inequality (best facet) \\
\hline \\[-1.8ex]
const & 11.875$^{}$ & 12.566$^{}$ & 40.365$^{***}$ & 48.337$^{***}$ \\
  & (9.882) & (9.231) & (9.665) & (8.943) \\
 EV: pay, economic & & & & -0.558$^{***}$ \\
  & & & & (0.124) \\
 EV: supportive environment & & 0.434$^{**}$ & & \\
  & & (0.164) & & \\
sustainability score & 0.318$^{**}$ & & -0.416$^{***}$ & \\
  & (0.157) & & (0.154) & \\
 urbanPop\_log scaled & 0.440$^{***}$ & 0.383$^{***}$ & 0.284$^{**}$ & 0.182$^{}$ \\
  & (0.129) & (0.130) & (0.126) & (0.109) \\
\hline \\[-1.8ex]
 Observations & 50 & 50 & 50 & 50 \\
 $R^2$ & 0.310 & 0.348 & 0.172 & 0.332 \\
 Adjusted $R^2$ & 0.281 & 0.320 & 0.137 & 0.304 \\
 Residual Std. Error & 20.972(df = 47) & 20.391(df = 47) & 20.510(df = 47) & 18.419(df = 47)  \\
 F Statistic & 10.561$^{***}$ (df = 2.0; 47.0) & 12.528$^{***}$ (df = 2.0; 47.0) & 4.884$^{**}$ (df = 2.0; 47.0) & 11.696$^{***}$ (df = 2.0; 47.0) \\
\hline
\hline \\[-1.8ex]
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}
\caption{OLS models predicting state GDP and Gini coefficient (both logged). Running stepAIC reveals that the full model is the minimal model in both cases. All variables are scaled between 0 and 100 to aid in interpretability.}
\label{tab:gdp_and_gini_combined}
\end{table}

\begin{table}[!htbp] \centering \small
\begin{tabular}{@{\extracolsep{5pt}}lcccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
\\[-1.8ex] & GDP (control) & GDP (full) & Gini (control) & Gini (full) \\
\hline \\[-1.8ex]
const & 19.815$^{**}$ & 11.875$^{}$ & 29.990$^{***}$ & 40.365$^{***}$ \\
  & (9.354) & (9.882) & (9.431) & (9.665) \\
 urbanPop\_log scaled & 0.511$^{***}$ & 0.440$^{***}$ & 0.191$^{}$ & 0.284$^{**}$ \\
  & (0.128) & (0.129) & (0.129) & (0.126) \\
 sustainability score scaled & & 0.318$^{**}$ & & -0.416$^{***}$ \\
  & & (0.157) & & (0.154) \\
\hline \\[-1.8ex]
 Observations & 50 & 50 & 50 & 50 \\
 $R^2$ & 0.250 & 0.310 & 0.044 & 0.172 \\
 Adjusted $R^2$ & 0.235 & 0.281 & 0.024 & 0.137 \\
 Residual Std. Error & 21.635(df = 48) & 20.972(df = 47) & 21.812(df = 48) & 20.510(df = 47)  \\
 F Statistic & 16.011$^{***}$ (df = 1.0; 48.0) & 10.561$^{***}$ (df = 2.0; 47.0) & 2.192$^{}$ (df = 1.0; 48.0) & 4.884$^{**}$ (df = 2.0; 47.0) \\
\hline
\hline \\[-1.8ex]
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}
\caption{OLS models predicting state GDP and Gini coefficient (both logged). The control model only uses the controls as explanatory variables (urban density), while the full model uses the composite sustainability score $S(u)$ in addition to the controls. Running stepAIC reveals that the full model is the minimal model in both cases. All variables are scaled between 0 and 100 to aid in interpretability.}
\label{tab:gdp_and_gini_su}
\end{table}


\begin{table}[!htbp] \centering \small
\begin{tabular}{@{\extracolsep{5pt}}lcccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
\\[-1.8ex] & GDP (control) & GDP (full) & Gini (control) & Gini (full) \\
\hline \\[-1.8ex]
 const & 19.815$^{**}$ & 12.566$^{}$ & 29.990$^{***}$ & 48.337$^{***}$ \\
  & (9.354) & (9.231) & (9.431) & (8.943) \\
 EV: pay, economic & & & & -0.558$^{***}$ \\
  & & & & (0.124) \\
 EV: supportive environment & & 0.434$^{**}$ & & \\
  & & (0.164) & & \\
 urbanPop\_log scaled & 0.511$^{***}$ & 0.383$^{***}$ & 0.191$^{}$ & 0.182$^{}$ \\
  & (0.128) & (0.130) & (0.129) & (0.109) \\
\hline \\[-1.8ex]
 Observations & 50 & 50 & 50 & 50 \\
 $R^2$ & 0.250 & 0.348 & 0.044 & 0.332 \\
 Adjusted $R^2$ & 0.235 & 0.320 & 0.024 & 0.304 \\
 Residual Std. Error & 21.635(df = 48) & 20.391(df = 47) & 21.812(df = 48) & 18.419(df = 47)  \\
 F Statistic & 16.011$^{***}$ (df = 1.0; 48.0) & 12.528$^{***}$ (df = 2.0; 47.0) & 2.192$^{}$ (df = 1.0; 48.0) & 11.696$^{***}$ (df = 2.0; 47.0) \\
\hline
\hline \\[-1.8ex]
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}
\caption{OLS models predicting state GDP and Gini coefficient (both logged). The control model only uses the controls as explanatory variables (urban density), while the full model uses relevant sustainability goals --- supportive environment for GDP and pay for Gini. Running stepAIC reveals that the full model is the minimal model in both cases. All variables are scaled between 0 and 100 to aid in interpretability.}
\label{tab:gdp_and_gini_sug}
\end{table}


\begin{table}[!htbp] \centering
\scriptsize
\begin{tabular}{@{\extracolsep{5pt}}lccccccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
\\[-1.8ex] & composite & health & education & gender & finance & infrastructure & supportive \\
\hline \\[-1.8ex]
 const & 112.893$^{**}$ & 1.003$^{}$ & -1.765$^{}$ & 149.950$^{***}$ & 119.246$^{***}$ & 117.062$^{***}$ & 23.906$^{**}$ \\
  & (45.057) & (20.974) & (13.844) & (43.078) & (42.607) & (39.869) & (11.370) \\
 cultural
tightness & -2.043$^{**}$ & & & -1.940$^{**}$ & -2.093$^{**}$ & -2.216$^{***}$ & -0.619$^{***}$ \\
  & (0.866) & & & (0.821) & (0.796) & (0.766) & (0.217) \\
 cultural tightness *
wealth & 2.274$^{**}$ & & 0.242$^{*}$ & 2.058$^{**}$ & 2.171$^{***}$ & 2.436$^{***}$ & 0.673$^{***}$ \\
  & (0.859) & & (0.143) & (0.811) & (0.790) & (0.761) & (0.216) \\
 inequality & -3.527$^{***}$ & & -0.934$^{*}$ & -1.690$^{**}$ & -4.048$^{***}$ & -3.131$^{***}$ & -0.944$^{***}$ \\
  & (0.887) & & (0.488) & (0.676) & (0.896) & (0.785) & (0.224) \\
 lgbtq
travel & 1.724$^{***}$ & 0.981$^{***}$ & 1.345$^{***}$ & & 2.185$^{***}$ & 1.346$^{***}$ & 0.431$^{***}$ \\
  & (0.452) & (0.361) & (0.499) & & (0.414) & (0.400) & (0.114) \\
 lgbtq travel*
creativity & & & & -0.282$^{*}$ & 1.398$^{**}$ & & 0.085$^{}$ \\
  & & & & (0.160) & (0.569) & & (0.052) \\
 lgbtq travel*
urbanization & -3.016$^{***}$ & -1.294$^{**}$ & -1.704$^{**}$ & & -4.056$^{***}$ & -2.599$^{***}$ & -0.784$^{***}$ \\
  & (0.745) & (0.517) & (0.753) & & (0.726) & (0.659) & (0.187) \\
 total reviews*
lgbtq travel & 8.799$^{***}$ & & & & 5.391$^{**}$ & 9.236$^{***}$ & 2.043$^{***}$ \\
  & (2.702) & & & & (1.993) & (2.391) & (0.653) \\
 total reviews*
urbanization & -3.113$^{*}$ & & & & & -3.249$^{**}$ & -0.609$^{}$ \\
  & (1.802) & & & & & (1.595) & (0.444) \\
 total reviews*creativity & -5.469$^{**}$ & & & & -5.235$^{**}$ & -5.843$^{***}$ & -1.399$^{**}$ \\
  & (2.159) & & & & (1.975) & (1.910) & (0.547) \\
 urbanization & & 0.410$^{}$ & & & & & \\
  & & (0.293) & & & & & \\
 urbanization*
creativity & 0.420$^{**}$ & & & & -0.793$^{}$ & 0.411$^{**}$ & \\
  & (0.204) & & & & (0.549) & (0.180) & \\
 urbanization*
wealth & 3.454$^{***}$ & 0.466$^{**}$ & 1.825$^{**}$ & 0.542$^{**}$ & 4.444$^{***}$ & 2.936$^{***}$ & 0.903$^{***}$ \\
  & (0.826) & (0.195) & (0.780) & (0.265) & (0.935) & (0.731) & (0.203) \\
 wealth & -0.589$^{***}$ & -0.185$^{}$ & -0.351$^{**}$ & -0.563$^{***}$ & -0.446$^{***}$ & -0.456$^{***}$ & -0.143$^{***}$ \\
  & (0.139) & (0.117) & (0.144) & (0.132) & (0.130) & (0.123) & (0.035) \\
\hline \\[-1.8ex]
 Observations & 50 & 50 & 50 & 50 & 50 & 50 & 50 \\
 $R^2$ & 0.572 & 0.302 & 0.359 & 0.438 & 0.661 & 0.605 & 0.570 \\
 Adjusted $R^2$ & 0.449 & 0.222 & 0.269 & 0.360 & 0.562 & 0.490 & 0.445 \\
 Residual Std. Error & 15.457(df = 38) & 16.999(df = 44) & 18.754(df = 43) & 17.024(df = 43) & 14.167(df = 38) & 13.677(df = 38) & 3.874(df = 38)  \\
 F Statistic & 4.624$^{***}$  & 3.801$^{***}$  & 4.012$^{***}$ & 5.590$^{***}$ & 6.726$^{***}$ & 5.284$^{***}$  & 4.578$^{***}$ \\
 & (df = 11.0; 38.0) & (df = 5.0; 44.0) & (df = 6.0; 43.0) & (df = 6.0; 43.0) & (df = 11.0; 38.0) & (df = 11.0; 38.0) & (df = 11.0; 38.0) \\
\hline
\hline \\[-1.8ex]
\textit{Note:} & \multicolumn{7}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}
\caption{StepAIC models for predicting sustainability scores for the composite sustainability score and the six individual goals.}
\label{tab:6goals}
\end{table}


% non-interaction table

\begin{table}[!htbp] \centering
\scriptsize
\begin{tabular}{@{\extracolsep{5pt}}lccccccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
\\[-1.8ex] & composite & health & education & gender & finance & infra & supp. env \\
\hline \\[-1.8ex]
 const & -6.955$^{**}$ & 30.933$^{***}$ & 22.372$^{**}$ & 20.590$^{**}$ & 149.950$^{***}$ & 48.058$^{**}$ & 10.911$^{}$ \\
  & (2.769) & (7.691) & (10.931) & (9.631) & (43.078) & (20.660) & (9.337) \\
 creativity & 0.073$^{*}$ & & 0.228$^{}$ & & & 0.462$^{***}$ & 0.299$^{**}$ \\
  & (0.036) & & (0.151) & & & (0.154) & (0.133) \\
 cultural
tightness & & & & & -1.940$^{**}$ & & \\
  & & & & & (0.821) & & \\
 cultural tightness *
wealth & 0.067$^{**}$ & 0.187$^{}$ & 1.259$^{**}$ & & 2.058$^{**}$ & 0.300$^{*}$ & 0.234$^{**}$ \\
  & (0.030) & (0.121) & (0.553) & & (0.811) & (0.153) & (0.111) \\
 inequality & -0.100$^{***}$ & -0.428$^{***}$ & -0.335$^{***}$ & -0.319$^{**}$ & -0.563$^{***}$ & -0.352$^{**}$ & -0.337$^{***}$ \\
  & (0.031) & (0.126) & (0.122) & (0.130) & (0.132) & (0.150) & (0.107) \\
 lgbtq
travel & 0.051$^{}$ & & 1.077$^{**}$ & & & 0.379$^{**}$ & \\
  & (0.035) & & (0.500) & & & (0.150) & \\
 lgbtq travel*
creativity & & & & & -0.282$^{*}$ & & \\
  & & & & & (0.160) & & \\
 lgbtq travel*
cultural tightness & & & -1.314$^{*}$ & 0.291$^{*}$ & & & \\
  & & & (0.665) & (0.152) & & & \\
 urbanization & & & & & & -1.001$^{***}$ & \\
  & & & & & & (0.371) & \\
 urbanization*
creativity & & 0.414$^{***}$ & & & & & \\
  & & (0.100) & & & & & \\
 urbanization*
wealth & & & & 0.347$^{***}$ & 0.542$^{**}$ & 1.443$^{**}$ & 0.214$^{*}$ \\
  & & & & (0.112) & (0.265) & (0.658) & (0.117) \\
 wealth & & & -0.595$^{}$ & & -1.690$^{**}$ & -0.931$^{**}$ & \\
  & & & (0.381) & & (0.676) & (0.451) & \\
\hline \\[-1.8ex]
 Observations & 50 & 50 & 50 & 50 & 50 & 50 & 50 \\
 $R^2$ & 0.334 & 0.317 & 0.323 & 0.261 & 0.438 & 0.463 & 0.392 \\
 Adjusted $R^2$ & 0.275 & 0.272 & 0.229 & 0.213 & 0.360 & 0.374 & 0.338 \\
 Residual Std. Error & 4.430(df = 45) & 17.759(df = 46) & 16.928(df = 43) & 19.467(df = 46) & 17.024(df = 43) & 16.947(df = 42) & 15.590(df = 45)  \\
 F Statistic & 5.640$^{***}$ (df = 4.0; 45.0) & 7.105$^{***}$ (df = 3.0; 46.0) & 3.423$^{***}$ (df = 6.0; 43.0) & 5.417$^{***}$ (df = 3.0; 46.0) & 5.590$^{***}$ (df = 6.0; 43.0) & 5.180$^{***}$ (df = 7.0; 42.0) & 7.243$^{***}$ (df = 4.0; 45.0) \\
\hline
\hline \\[-1.8ex]
\textit{Note:} & \multicolumn{7}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}
\caption{StepAIC models for predicting sustainability scores for the seven dimensions without interaction variables.}
\label{tab:6goals_no_interaction}
\end{table}

% OLD non-interaction table




\begin{table}[!htbp] \centering \scriptsize
\begin{tabular}{@{\extracolsep{5pt}}lcccccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
\\[-1.8ex] & health & education & gender & financial & support & supportive \\
\\[-1.8ex] & & & equality & benefit &  infrastructure & supportive \\
\hline \\[-1.8ex]
const & 34.521$^{***}$ & 42.681$^{***}$ & 26.720$^{***}$ & 54.279$^{***}$ & 45.890$^{***}$ & 25.595$^{***}$ \\
  & (5.471) & (7.964) & (8.824) & (5.662) & (12.564) & (6.739) \\
 E\_2a\_gdp\_log scaled & & 0.282$^{***}$ & 0.182$^{}$ & & & 0.180$^{*}$ \\
  & & (0.102) & (0.124) & & & (0.095) \\
 P\_2a\_freedomIndex\_log scaled & & & & & -0.189$^{}$ & \\
  & & & & & (0.127) & \\
 P\_3c\_giniCoefficient\_log scaled & -0.281$^{**}$ & -0.217$^{*}$ & -0.256$^{}$ & -0.522$^{***}$ & & -0.179$^{}$ \\
  & (0.125) & (0.114) & (0.153) & (0.117) & & (0.117) \\
 S\_1b\_lgbtqTravelIndex\_log scaled & & & & & 0.341$^{**}$ & \\
  & & & & & (0.133) & \\
 S\_9a\_urbanPop\_log scaled & & & & & -0.333$^{**}$ & \\
  & & & & & (0.137) & \\
 population\_2019\_log scaled & -1.475$^{***}$ & & -0.874$^{**}$ & & -1.438$^{***}$ & -1.175$^{***}$ \\
  & (0.325) & & (0.434) & & (0.347) & (0.331) \\
 total reviews\_log scaled & 1.709$^{***}$ & & 1.051$^{**}$ & & 1.660$^{***}$ & 1.294$^{***}$ \\
  & (0.301) & & (0.413) & & (0.379) & (0.316) \\
\hline \\[-1.8ex]
 Observations & 50 & 50 & 50 & 50 & 50 & 50 \\
 $R^2$ & 0.478 & 0.196 & 0.309 & 0.293 & 0.504 & 0.472 \\
 Adjusted $R^2$ & 0.444 & 0.162 & 0.248 & 0.278 & 0.447 & 0.425 \\
 Residual Std. Error & 15.527(df = 46) & 17.649(df = 47) & 19.028(df = 45) & 18.078(df = 48) & 15.920(df = 44) & 14.531(df = 45)  \\
 F Statistic & 14.020$^{***}$ & 5.726$^{***}$  & 5.038$^{***}$ & 19.872$^{***}$  & 8.935$^{***}$  & 10.037$^{***}$  \\
 & (df = 3.0; 46.0) & (df = 2.0; 47.0) &  (df = 4.0; 45.0) &  (df = 1.0; 48.0) & (df = 5.0; 44.0) & (df = 4.0; 45.0) \\
\hline
\hline \\[-1.8ex]
\textit{Note:} & \multicolumn{6}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}
\caption{StepAIC models for predicting sustainability scores for the six goals.}
\label{tab:6goals_no_interaction}
\end{table}


\begin{table}[!htbp] \centering \small
\begin{tabular}{@{\extracolsep{5pt}}lccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
\\[-1.8ex] & health & education & gender \\
\hline \\[-1.8ex]
 Creativity Index  & 0.002$^{*}$ & & 0.002$^{*}$ \\
  & (0.001) & & (0.001) \\
 E\_1b\_occupationEnterprising & & 5.040$^{**}$ & \\
  & & (2.299) & \\
 E\_1f\_occupationsRealistic & & & -3.511$^{*}$ \\
  & & & (1.917) \\
 E\_2a\_gdp & 0.000$^{**}$ & 0.000$^{***}$ & 0.000$^{***}$ \\
  & (0.000) & (0.000) & (0.000) \\
 P\_3c\_giniCoefficient & -4.808$^{***}$ & -2.861$^{**}$ & -4.228$^{**}$ \\
  & (1.674) & (1.313) & (1.618) \\
 P\_4b\_cultural tightness  & 0.006$^{**}$ & & \\
  & (0.003) & & \\
 S\_2a\_collectivism & -0.005$^{**}$ & & \\
  & (0.002) & & \\
 S\_5a\_violentCrimes & -0.000$^{}$ & -0.000$^{**}$ & -0.000$^{*}$ \\
  & (0.000) & (0.000) & (0.000) \\
 S\_6b\_religiousModerately & -0.020$^{**}$ & & \\
  & (0.009) & & \\
 S\_8a\_educBachelor & -0.024$^{***}$ & -0.021$^{**}$ & -0.033$^{***}$ \\
  & (0.008) & (0.009) & (0.011) \\
 S\_9b\_fiveThirtyEightUrbanIndex & 0.116$^{***}$ & & \\
  & (0.041) & & \\
 const & 2.216$^{***}$ & 1.055$^{*}$ & 3.777$^{***}$ \\
  & (0.741) & (0.608) & (1.129) \\
\hline \\[-1.8ex]
 Observations & 50 & 50 & 50 \\
 $R^2$ & 0.526 & 0.332 & 0.364 \\
 Adjusted $R^2$ & 0.420 & 0.256 & 0.275 \\
 Residual Std. Error & 0.159(df = 40) & 0.166(df = 44) & 0.187(df = 43)  \\
 F Statistic & 4.941$^{***}$ (df = 9.0; 40.0) & 4.380$^{***}$ (df = 5.0; 44.0) & 4.098$^{***}$ (df = 6.0; 43.0) \\
\hline
\hline \\[-1.8ex]
\textit{Note:} & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}
\caption{\todo{this needs to be done with the subset of predictors discussed in the meeting} StepAIC models for predicting sustainability scores for health, education, and equality with different state socio-economic variables.}
\label{tab:6goals_old}
\end{table}


\begin{table}[!htbp] \centering
\begin{tabular}{@{\extracolsep{5pt}}lccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
\\[-1.8ex] & pay & work environment & supportive environment \\
\hline \\[-1.8ex]
 Creativity Index  & & 0.002$^{**}$ & 0.002$^{**}$ \\
  & & (0.001) & (0.001) \\
 E\_1b\_occupationEnterprising & 6.077$^{**}$ & & \\
  & (2.724) & & \\
 E\_1f\_occupationsRealistic & 3.440$^{*}$ & & -3.055$^{**}$ \\
  & (1.941) & & (1.499) \\
 E\_2a\_gdp & 0.000$^{**}$ & & 0.000$^{***}$ \\
  & (0.000) & & (0.000) \\
 P\_3c\_giniCoefficient & -4.976$^{***}$ & & -4.709$^{***}$ \\
  & (1.400) & & (1.346) \\
 P\_4b\_cultural tightness  & & & 0.003$^{}$ \\
  & & & (0.002) \\
 S\_1b\_lgbtqTravelIndex & & 0.014$^{*}$ & \\
  & & (0.008) & \\
 S\_2a\_collectivism & -0.003$^{}$ & & \\
  & (0.002) & & \\
 S\_5a\_violentCrimes & -0.000$^{**}$ & -0.000$^{**}$ & -0.000$^{**}$ \\
  & (0.000) & (0.000) & (0.000) \\
 S\_6b\_religiousModerately & -0.021$^{**}$ & -0.017$^{**}$ & \\
  & (0.008) & (0.008) & \\
 S\_8a\_educBachelor & -0.037$^{***}$ & -0.010$^{}$ & -0.029$^{***}$ \\
  & (0.009) & (0.007) & (0.008) \\
 S\_9b\_fiveThirtyEightUrbanIndex & 0.051$^{}$ & & \\
  & (0.034) & & \\
 const & 1.324$^{}$ & 0.970$^{***}$ & 3.489$^{***}$ \\
  & (1.174) & (0.342) & (0.875) \\
\hline \\[-1.8ex]
 Observations & 50 & 50 & 50 \\
 $R^2$ & 0.620 & 0.464 & 0.511 \\
 Adjusted $R^2$ & 0.535 & 0.403 & 0.430 \\
 Residual Std. Error & 0.145(df = 40) & 0.165(df = 44) & 0.145(df = 42)  \\
 F Statistic & 7.261$^{***}$ (df = 9.0; 40.0) & 7.625$^{***}$ (df = 5.0; 44.0) & 6.279$^{***}$ (df = 7.0; 42.0) \\
\hline
\hline \\[-1.8ex]
\textit{Note:} & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}
\caption{\todo{this needs to be done with the subset of predictors discussed in the meeting} StepAIC models for predicting sustainability scores for pay, work environment, and supportive environment with different state socio-economic variables.}
\label{tab:6goals_second_old}
\end{table}

\end{comment}



% \begin{table}[t] \centering \small
% \begin{tabular}{@{\extracolsep{5pt}}lccc}
% \\[-1.8ex]\hline
% \hline \\[-1.8ex]
% & \multicolumn{3}{c}{\textit{GDP (logged)}} \
% \cr \cline{3-4}
% \\[-1.8ex] & controls & full model & stepAIC model \\
% \hline \\[-1.8ex]
%  supportive environment & & 0.521$^{*}$ & 0.729$^{***}$ \\
%   & & (0.292) & (0.246) \\
%  health & & -0.344$^{}$ & -0.306$^{}$ \\
%   & & (0.274) & (0.210) \\
%  education & & 0.176$^{}$ & \\
%   & & (0.203) & \\
%  gender & & 0.203$^{}$ & \\
%   & & (0.230) & \\
%  pay & & -0.112$^{}$ & \\
%   & & (0.163) & \\
%  work environment & & -0.350$^{*}$ & -0.275$^{}$ \\
%   & & (0.186) & (0.172) \\
%  const & 20.262$^{***}$ & 19.222$^{***}$ & 18.925$^{***}$ \\
%   & (1.792) & (1.865) & (1.834) \\
%  population\_2019\_log & -0.752$^{***}$ & -0.677$^{***}$ & -0.645$^{***}$ \\
%   & (0.134) & (0.146) & (0.142) \\
%  reviews x population log & 0.055$^{***}$ & 0.049$^{***}$ & 0.049$^{***}$ \\
%   & (0.013) & (0.012) & (0.012) \\
%  total reviews\_log & -0.593$^{***}$ & -0.513$^{**}$ & -0.543$^{***}$ \\
%   & (0.191) & (0.193) & (0.187) \\
% \hline \\[-1.8ex]
%  Observations & 50 & 50 & 50 \\
%  $R^2$ & 0.441 & 0.563 & 0.537 \\
%  Adjusted $R^2$ & 0.404 & 0.465 & 0.473 \\
%  Residual Std. Error & 0.146(df = 46) & 0.138(df = 40) & 0.137(df = 43)  \\
%  F Statistic & 12.086$^{***}$ (df = 3.0; 46.0) & 5.723$^{***}$ (df = 9.0; 40.0) & 8.322$^{***}$ (df = 6.0; 43.0) \\
% \hline
% \hline \\[-1.8ex]
% \textit{Note:} & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
% \end{tabular}
% \caption{OLS models predicting state GDP (logged). The control model only uses the controls as explanatory variables, while the full model uses the 6 sustainability scores in addition to the controls. Finally, the stepAIC model is obtained by obtaining the minimal set of variables with the lowest AIC.}
% \label{tab:gdp}
% \end{table}

% \begin{table}[!htbp] \centering
% \begin{tabular}{@{\extracolsep{5pt}}lccc}
% \\[-1.8ex]\hline
% \hline \\[-1.8ex]
% & \multicolumn{3}{c}{\textit{GDP (logged)}} \
% \cr \cline{3-4}
% \\[-1.8ex] & (1) & (2) & (3) \\
% \hline \\[-1.8ex]
% const & 11.938$^{***}$ & 12.671$^{***}$ & 12.627$^{***}$ \\
% & (0.657) & (0.629) & (0.603) \\
%  EV: education & & 0.056$^{}$ & \\
%   & & (0.198) & \\
%  EV: gender diversity & & 0.244$^{}$ & \\
%   & & (0.221) & \\
%  EV: health & & -0.413$^{}$ & -0.405$^{**}$ \\
%   & & (0.247) & (0.196) \\
%  EV: pay, economic & & -0.124$^{}$ & \\
%   & & (0.157) & \\
%  EV: supportive environment & & 0.903$^{***}$ & 1.061$^{***}$ \\
%   & & (0.291) & (0.252) \\
%  EV: work environment & & -0.357$^{*}$ & -0.303$^{}$ \\
%   & & (0.201) & (0.190) \\
%  S\_9a\_urbanPop & -0.012$^{}$ & -0.024$^{***}$ & -0.024$^{***}$ \\
%   & (0.009) & (0.009) & (0.009) \\
%  reviews x urban pop log & 0.003$^{**}$ & 0.004$^{***}$ & 0.004$^{***}$ \\
%   & (0.001) & (0.001) & (0.001) \\
%  total reviews\_log & -0.219$^{**}$ & -0.306$^{***}$ & -0.299$^{***}$ \\
%   & (0.089) & (0.081) & (0.079) \\
% \hline \\[-1.8ex]
%  Observations & 50 & 50 & 50 \\
%  $R^2$ & 0.343 & 0.586 & 0.566 \\
%  Adjusted $R^2$ & 0.301 & 0.493 & 0.505 \\
%  Residual Std. Error & 0.158(df = 46) & 0.135(df = 40) & 0.133(df = 43)  \\
%  F Statistic & 8.023$^{***}$ (df = 3.0; 46.0) & 6.298$^{***}$ (df = 9.0; 40.0) & 9.329$^{***}$ (df = 6.0; 43.0) \\
% \hline
% \hline \\[-1.8ex]
% \textit{Note:} & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
% \end{tabular}
% \caption{OLS models predicting state GDP (logged). The control model only uses the controls as explanatory variables (total reviews, urban density, and their interaction), while the full model uses the 6 sustainability scores in addition to the controls. Finally, the stepAIC model is obtained by obtaining the minimal set of variables with the lowest AIC.}
% \label{tab:gdp_urban}
% \end{table}

% \begin{table}[!htbp] \centering
% \begin{tabular}{@{\extracolsep{5pt}}lccc}
% \\[-1.8ex]\hline
% \hline \\[-1.8ex]
% & \multicolumn{3}{c}{\textit{GDP (logged)}} \
% \cr \cline{3-4}
% \\[-1.8ex] & (1) & (2) & (3) \\
% \hline \\[-1.8ex]
%  const & 10.652$^{***}$ & 10.614$^{***}$ & 10.779$^{***}$ \\
%  & (0.154) & (0.189) & (0.060) \\
%  EV: education & & 0.128$^{}$ & \\
%   & & (0.243) & \\
%  EV: gender diversity & & 0.076$^{}$ & \\
%   & & (0.271) & \\
%  EV: health & & -0.285$^{}$ & \\
%   & & (0.304) & \\
%  EV: pay, economic & & -0.168$^{}$ & -0.254$^{*}$ \\
%   & & (0.195) & (0.133) \\
%  EV: supportive environment & & 0.908$^{***}$ & 0.896$^{***}$ \\
%   & & (0.331) & (0.246) \\
%  EV: work environment & & -0.307$^{}$ & -0.309$^{}$ \\
%   & & (0.225) & (0.197) \\
%  total reviews\_log & 0.029$^{}$ & 0.018$^{}$ & \\
%   & (0.019) & (0.022) & \\
% \hline \\[-1.8ex]
%  Observations & 50 & 50 & 50 \\
%  $R^2$ & 0.047 & 0.327 & 0.299 \\
%  Adjusted $R^2$ & 0.027 & 0.215 & 0.254 \\
%  Residual Std. Error & 0.187(df = 48) & 0.168(df = 42) & 0.163(df = 46)  \\
%  F Statistic & 2.367$^{}$ (df = 1.0; 48.0) & 2.912$^{**}$ (df = 7.0; 42.0) & 6.553$^{***}$ (df = 3.0; 46.0) \\
% \hline
% \hline \\[-1.8ex]
% \textit{Note:} & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
% \end{tabular}
% \caption{OLS models predicting state GDP (logged). The control model only uses the controls as explanatory variables (only glassdoor reviews), while the full model uses the 6 sustainability scores in addition to the controls. Finally, the stepAIC model is obtained by obtaining the minimal set of variables with the lowest AIC.}
% \label{tab:gdp_reviews}
% \end{table}

% \begin{table}[!htbp] \centering
% \begin{tabular}{@{\extracolsep{5pt}}lccc}
% \\[-1.8ex]\hline
% \hline \\[-1.8ex]
% & \multicolumn{3}{c}{\textit{GDP (logged)}} \
% \cr \cline{3-4}
% \\[-1.8ex] & (1) & (2) & (3) \\
% \hline \\[-1.8ex]
%  EV: education & & 0.165$^{}$ & \\
%   & & (0.222) & \\
%  EV: gender diversity & & 0.143$^{}$ & \\
%   & & (0.248) & \\
%  EV: health & & -0.462$^{}$ & -0.473$^{**}$ \\
%   & & (0.275) & (0.213) \\
%  EV: pay, economic & & -0.085$^{}$ & \\
%   & & (0.160) & \\
%  EV: supportive environment & & 0.681$^{**}$ & 0.774$^{***}$ \\
%   & & (0.308) & (0.230) \\
%  EV: work environment & & -0.160$^{}$ & \\
%   & & (0.209) & \\
%  S\_9a\_urbanPop & 0.007$^{***}$ & 0.005$^{***}$ & 0.005$^{***}$ \\
%   & (0.002) & (0.002) & (0.002) \\
%  const & 10.404$^{***}$ & 10.378$^{***}$ & 10.382$^{***}$ \\
%   & (0.121) & (0.142) & (0.110) \\
% \hline \\[-1.8ex]
%  Observations & 50 & 50 & 50 \\
%  $R^2$ & 0.254 & 0.440 & 0.418 \\
%  Adjusted $R^2$ & 0.238 & 0.347 & 0.380 \\
%  Residual Std. Error & 0.165(df = 48) & 0.153(df = 42) & 0.149(df = 46)  \\
%  F Statistic & 16.329$^{***}$ (df = 1.0; 48.0) & 4.715$^{***}$ (df = 7.0; 42.0) & 11.009$^{***}$ (df = 3.0; 46.0) \\
% \hline
% \hline \\[-1.8ex]
% \textit{Note:} & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
% \end{tabular}
% \caption{OLS models predicting state GDP (logged). The control model only uses the controls as explanatory variables (only urban population), while the full model uses the 6 sustainability scores in addition to the controls. Finally, the stepAIC model is obtained by obtaining the minimal set of variables with the lowest AIC.}
% \label{tab:gdp_oly_urban}
% \end{table}

% \begin{table}[!htbp] \centering
% \begin{tabular}{@{\extracolsep{5pt}}lccc}
% \\[-1.8ex]\hline
% \hline \\[-1.8ex]
% & \multicolumn{3}{c}{\textit{Gini (logged)}} \
% \cr \cline{3-4}
% \\[-1.8ex] & control model & full model & stepAIC model \\
% \hline \\[-1.8ex]
%  suportive environment & & 0.028$^{}$ & \\
%   & & (0.071) & \\
%  health & & -0.025$^{}$ & \\
%   & & (0.067) & \\
%  education & & -0.008$^{}$ & \\
%   & & (0.049) & \\
%  gender & & 0.017$^{}$ & \\
%   & & (0.056) & \\
%  pay & & -0.066$^{}$ & -0.071$^{***}$ \\
%   & & (0.040) & (0.023) \\
%  work environment & & -0.020$^{}$ & \\
%   & & (0.045) & \\
%  const & -1.324$^{***}$ & -1.142$^{**}$ & -1.016$^{***}$ \\
%   & (0.422) & (0.453) & (0.076) \\
%  population\_2019\_log & 0.043$^{}$ & 0.028$^{}$ & 0.018$^{***}$ \\
%   & (0.032) & (0.036) & (0.005) \\
%  reviews x population log & -0.000$^{}$ & -0.001$^{}$ & \\
%   & (0.003) & (0.003) & \\
%  total reviews\_log & -0.004$^{}$ & 0.008$^{}$ & \\
%   & (0.045) & (0.047) & \\
% \hline \\[-1.8ex]
%  Observations & 50 & 50 & 50 \\
%  $R^2$ & 0.354 & 0.462 & 0.453 \\
%  Adjusted $R^2$ & 0.312 & 0.341 & 0.429 \\
%  Residual Std. Error & 0.034(df = 46) & 0.034(df = 40) & 0.031(df = 47)  \\
%  F Statistic & 8.402$^{***}$ (df = 3.0; 46.0) & 3.822$^{***}$ (df = 9.0; 40.0) & 19.428$^{***}$ (df = 2.0; 47.0) \\
% \hline
% \hline \\[-1.8ex]
% \textit{Note:} & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
% \end{tabular}
% \caption{OLS models predicting state Gini coefficient (logged). The control model only uses the controls as explanatory variables, while the full model uses the 6 sustainability scores in addition to the controls. Finally, the stepAIC model is obtained by obtaining the minimal set of variables with the lowest AIC.}
% \label{tab:gini}
% \end{table}

% \begin{table}[!htbp] \centering \small
% \begin{tabular}{@{\extracolsep{5pt}}lccc}
% \\[-1.8ex]\hline
% \hline \\[-1.8ex]
% & \multicolumn{3}{c}{\textit{Gini (logged)}} \
% \cr \cline{3-4}
% \\[-1.8ex] & (1) & (2) & (3) \\
% \hline \\[-1.8ex]
%  const & -0.780$^{***}$ & -0.777$^{***}$ & -0.836$^{***}$ \\
%  & (0.148) & (0.158) & (0.031) \\
%  EV: education & & -0.006$^{}$ & \\
%   & & (0.050) & \\
%  EV: gender diversity & & 0.028$^{}$ & \\
%   & & (0.055) & \\
%  EV: health & & -0.042$^{}$ & \\
%   & & (0.062) & \\
%  EV: pay, economic & & -0.059$^{}$ & -0.081$^{***}$ \\
%   & & (0.039) & (0.023) \\
%  EV: supportive environment & & 0.021$^{}$ & \\
%   & & (0.073) & \\
%  EV: work environment & & -0.034$^{}$ & \\
%   & & (0.050) & \\
%  S\_9a\_urbanPop & -0.002$^{}$ & -0.001$^{}$ & \\
%   & (0.002) & (0.002) & \\
%  reviews x urban pop log & 0.000$^{}$ & 0.000$^{}$ & \\
%   & (0.000) & (0.000) & \\
%  total reviews\_log & 0.004$^{}$ & 0.006$^{}$ & 0.011$^{***}$ \\
%   & (0.020) & (0.020) & (0.003) \\
% \hline \\[-1.8ex]
%  Observations & 50 & 50 & 50 \\
%  $R^2$ & 0.301 & 0.454 & 0.427 \\
%  Adjusted $R^2$ & 0.255 & 0.331 & 0.402 \\
%  Residual Std. Error & 0.036(df = 46) & 0.034(df = 40) & 0.032(df = 47)  \\
%  F Statistic & 6.601$^{***}$ (df = 3.0; 46.0) & 3.700$^{***}$ (df = 9.0; 40.0) & 17.492$^{***}$ (df = 2.0; 47.0) \\
% \hline
% \hline \\[-1.8ex]
% \textit{Note:} & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
% \end{tabular}
% \caption{OLS models predicting state Gini coefficient (logged). The control model only uses the controls as explanatory variables (total reviews, urban density, and their interaction), while the full model uses the 6 sustainability scores in addition to the controls. Finally, the stepAIC model is obtained by obtaining the minimal set of variables with the lowest AIC.}
% \label{tab:gini_urban}
% \end{table}

% \begin{table}[!htbp] \centering
% \begin{tabular}{@{\extracolsep{5pt}}lccc}
% \\[-1.8ex]\hline
% \hline \\[-1.8ex]
% & \multicolumn{3}{c}{\textit{Gini (logged)}} \
% \cr \cline{3-4}
% \\[-1.8ex] & (1) & (2) & (3) \\
% \hline \\[-1.8ex]
% const & -0.894$^{***}$ & -0.851$^{***}$ & -0.836$^{***}$ \\
%   & (0.030) & (0.037) & (0.031) \\
%  EV: education & & -0.001$^{}$ & \\
%   & & (0.048) & \\
%  EV: gender diversity & & 0.029$^{}$ & \\
%   & & (0.054) & \\
%  EV: health & & -0.045$^{}$ & \\
%   & & (0.060) & \\
%  EV: pay, economic & & -0.060$^{}$ & -0.081$^{***}$ \\
%   & & (0.039) & (0.023) \\
%  EV: supportive environment & & 0.003$^{}$ & \\
%   & & (0.066) & \\
%  EV: work environment & & -0.020$^{}$ & \\
%   & & (0.044) & \\
%  total reviews\_log & 0.015$^{***}$ & 0.014$^{***}$ & 0.011$^{***}$ \\
%   & (0.004) & (0.004) & (0.003) \\
% \hline \\[-1.8ex]
%  Observations & 50 & 50 & 50 \\
%  $R^2$ & 0.274 & 0.449 & 0.427 \\
%  Adjusted $R^2$ & 0.259 & 0.358 & 0.402 \\
%  Residual Std. Error & 0.036(df = 48) & 0.033(df = 42) & 0.032(df = 47)  \\
%  F Statistic & 18.118$^{***}$ (df = 1.0; 48.0) & 4.897$^{***}$ (df = 7.0; 42.0) & 17.492$^{***}$ (df = 2.0; 47.0) \\
% \hline
% \hline \\[-1.8ex]
% \textit{Note:} & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
% \end{tabular}
% \caption{OLS models predicting state Gini coefficient (logged). The control model only uses the controls as explanatory variables (only glassdoor reviews), while the full model uses the 6 sustainability scores in addition to the controls. Finally, the stepAIC model is obtained by obtaining the minimal set of variables with the lowest AIC.}
% \label{tab:gini_reviews}
% \end{table}

% \begin{table}[!htbp] \centering
% \begin{tabular}{@{\extracolsep{5pt}}lccc}
% \\[-1.8ex]\hline
% \hline \\[-1.8ex]
% & \multicolumn{3}{c}{\textit{Gini (logged)}} \
% \cr \cline{3-4}
% \\[-1.8ex] & (1) & (2) & (3) \\
% \hline \\[-1.8ex]
%  EV: education & & -0.001$^{}$ & \\
%   & & (0.053) & \\
%  EV: gender diversity & & 0.044$^{}$ & \\
%   & & (0.059) & \\
%  EV: health & & -0.009$^{}$ & \\
%   & & (0.065) & \\
%  EV: pay, economic & & -0.108$^{***}$ & -0.104$^{***}$ \\
%   & & (0.038) & (0.023) \\
%  EV: supportive environment & & -0.035$^{}$ & \\
%   & & (0.073) & \\
%  EV: work environment & & 0.004$^{}$ & \\
%   & & (0.050) & \\
%  S\_9a\_urbanPop & 0.001$^{}$ & 0.001$^{}$ & 0.001$^{}$ \\
%   & (0.000) & (0.000) & (0.000) \\
%  const & -0.817$^{***}$ & -0.780$^{***}$ & -0.779$^{***}$ \\
%   & (0.030) & (0.034) & (0.027) \\
% \hline \\[-1.8ex]
%  Observations & 50 & 50 & 50 \\
%  $R^2$ & 0.049 & 0.342 & 0.331 \\
%  Adjusted $R^2$ & 0.029 & 0.232 & 0.303 \\
%  Residual Std. Error & 0.041(df = 48) & 0.036(df = 42) & 0.035(df = 47)  \\
%  F Statistic & 2.464$^{}$ (df = 1.0; 48.0) & 3.120$^{***}$ (df = 7.0; 42.0) & 11.649$^{***}$ (df = 2.0; 47.0) \\
% \hline
% \hline \\[-1.8ex]
% \textit{Note:} & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
% \end{tabular}
% \caption{OLS models predicting state Gini coefficient (logged). The control model only uses the controls as explanatory variables (only urban density), while the full model uses the 6 sustainability scores in addition to the controls. Finally, the stepAIC model is obtained by obtaining the minimal set of variables with the lowest AIC.}
% \label{tab:gini_only_urban}
% \end{table}



% \begin{comment}

% % Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% % Date and time: Fri, Jul 09, 2021 - 09:11:23 AM
% % Requires LaTeX packages: dcolumn 
% \begin{table*}[!htbp] \centering \scriptsize
%   \caption{Linear regressions.}
%   \label{table:gdp} 
% \begin{tabular}{@{\extracolsep{-30pt}}lD{.}{.}{-3} D{.}{.}{-3} D{.}{.}{-3} D{.}{.}{-3} D{.}{.}{-3} D{.}{.}{-3} } 
% \\[-1.8ex]\hline 
% \hline \\[-1.8ex] 
%  & \multicolumn{6}{c}{\textit{Dependent variable:}} \\ 
% \cline{2-7} 
% \\[-1.8ex] & \multicolumn{6}{c}{State-level} \\ 
%  & \multicolumn{1}{c}{GDP} & \multicolumn{1}{c}{GDP (stepAIC)} & \multicolumn{1}{c}{Inequality } & \multicolumn{1}{c}{Inequality   (stepAIC)} & \multicolumn{1}{c}{?} & \multicolumn{1}{c}{??} \\
% \\[-1.8ex] & \multicolumn{1}{c}{(1)} & \multicolumn{1}{c}{(2)} & \multicolumn{1}{c}{(3)} & \multicolumn{1}{c}{(4)} & \multicolumn{1}{c}{(5)} & \multicolumn{1}{c}{(6)}\\ 
% \hline \\[-1.8ex] 
%   $S(u)$ &  &  &  & -0.089^{**}$ $(0.044) &  &  \\ 
%     log(\#reviews) &  &  &  & -0.089^{**}$ $(0.044) &  &  \\ 
%     log(population) &  &  &  & -0.089^{**}$ $(0.044) &  &  \\ 
%     log(\#reviews)* log(population) &  &  &  & -0.089^{**}$ $(0.044) &  &  \\ 
%  % PERSONALITY\_neuroticism & -0.113^{***}$ $(0.038) &  &  & -0.098^{*}$ $(0.049) & -0.060^{**}$ $(0.027) &  \\ 
% %  PERSONALITY\_agreeableness &  &  &  &  &  & 0.039^{*}$ $(0.020) \\ 
% %   SOCIOECONOMIC\_no\_high\_school\_diploma &  & -0.110^{***}$ $(0.037) &  &  &  & -0.055^{**}$ $(0.025) \\ 
% %   PERSONALITY\_4b\_cultural\_tightness &  &  &  & 0.062$ $(0.044) &  &  \\ 
% %   SOCIOECONOMIC\_population\_2019 & 0.092^{***}$ $(0.034) & 0.102^{**}$ $(0.039) & 0.103^{***}$ $(0.030) & 0.051$ $(0.033) & 0.046^{*}$ $(0.023) & 0.042^{*}$ $(0.021) \\ 
% %   SOCIOECONOMIC\_density\_2015 &  & -0.069$ $(0.044) &  & -0.027$ $(0.039) &  &  \\ 
% %   POLITICAL\_p\_ideo\_diff & -0.187^{***}$ $(0.046) & -0.120^{*}$ $(0.062) & -0.091^{**}$ $(0.039) & -0.111^{*}$ $(0.065) &  &  \\ 
% %   population\_2019:\_density\_2015 &  &  &  & -0.096^{*}$ $(0.052) &  &  \\ 
% %   SOCIOECONOMIC\_gdp\_per\_capita\_2017 &  &  &  &  &  & -0.075$ $(0.055) \\ 
% %   Constant & 0.542^{***}$ $(0.030) & 0.563^{***}$ $(0.036) & 0.519^{***}$ $(0.029) & 0.532^{***}$ $(0.031) & 0.489^{***}$ $(0.024) & 0.491^{***}$ $(0.020) \\ 
%  \hline \\[-1.8ex] 
% Observations & \multicolumn{1}{c}{43} & \multicolumn{1}{c}{43} & \multicolumn{1}{c}{43} & \multicolumn{1}{c}{43} & \multicolumn{1}{c}{43} & \multicolumn{1}{c}{43} \\ 
% R$^{2}$ & \multicolumn{1}{c}{0.568} & \multicolumn{1}{c}{0.372} & \multicolumn{1}{c}{0.398} & \multicolumn{1}{c}{0.351} & \multicolumn{1}{c}{0.282} & \multicolumn{1}{c}{0.204} \\ 
% Adjusted R$^{2}$ & \multicolumn{1}{c}{0.523} & \multicolumn{1}{c}{0.306} & \multicolumn{1}{c}{0.368} & \multicolumn{1}{c}{0.221} & \multicolumn{1}{c}{0.227} & \multicolumn{1}{c}{0.120} \\ 
% Residual Std. Error & \multicolumn{1}{c}{0.192 (df = 38)} & \multicolumn{1}{c}{0.222 (df = 38)} & \multicolumn{1}{c}{0.187 (df = 40)} & \multicolumn{1}{c}{0.185 (df = 35)} & \multicolumn{1}{c}{0.151 (df = 39)} & \multicolumn{1}{c}{0.119 (df = 38)} \\ 
% F Statistic & \multicolumn{1}{c}{12.516$^{***}$ (df = 4; 38)} & \multicolumn{1}{c}{5.629$^{***}$ (df = 4; 38)} & \multicolumn{1}{c}{13.206$^{***}$ (df = 2; 40)} & \multicolumn{1}{c}{2.699$^{**}$ (df = 7; 35)} & \multicolumn{1}{c}{5.117$^{***}$ (df = 3; 39)} & \multicolumn{1}{c}{2.432$^{*}$ (df = 4; 38)} \\ 
% \hline 
% \hline \\[-1.8ex] 
% \textit{Note:}  & \multicolumn{6}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
% \end{tabular} 
% \end{table*} 

% \end{comment}




%%% previous table on predicting sustainability from state indicators

\begin{comment}
\begin{table}[t] 
\centering
\scriptsize
\begin{tabular}{@{\extracolsep{5pt}}lccccccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
\\[-1.8ex] & composite & health & education & gender & finance & infrastructure & supportive \\
\hline \\[-1.8ex]
 const & -2.167$^{}$ & 17.421$^{*}$ & 42.681$^{***}$ & 23.665$^{**}$ & 54.279$^{***}$ & 11.565$^{}$ & -3.021$^{}$ \\
  & (2.078) & (9.286) & (7.964) & (8.978) & (5.662) & (8.811) & (13.439) \\
 creativity & & 0.292$^{**}$ & & & & 0.387$^{**}$ & 0.347$^{***}$ \\
  & & (0.142) & & & & (0.148) & (0.124) \\
 cultural
tightness & & & & & & & 0.200$^{}$ \\
  & & & & & & & (0.122) \\
 inequality & -0.105$^{***}$ & -0.341$^{***}$ & -0.217$^{*}$ & -0.347$^{**}$ & -0.522$^{***}$ & & -0.294$^{**}$ \\
  & (0.035) & (0.120) & (0.114) & (0.151) & (0.117) & & (0.113) \\
 lgbtq
travel & & & & & & 0.397$^{***}$ & \\
  & & & & & & (0.146) & \\
 total
reviews & 0.065$^{**}$ & & & 0.262$^{*}$ & & & \\
  & (0.032) & & & (0.137) & & & \\
 urbanization & & 0.220$^{}$ & & & & -0.237$^{*}$ & \\
  & & (0.133) & & & & (0.140) & \\
 wealth & 0.062$^{**}$ & & 0.282$^{***}$ & 0.280$^{**}$ & & & 0.325$^{***}$ \\
  & (0.027) & & (0.102) & (0.118) & & & (0.109) \\
\hline \\[-1.8ex]
 Observations & 50 & 50 & 50 & 50 & 50 & 50 & 50 \\
 $R^2$ & 0.282 & 0.302 & 0.196 & 0.247 & 0.293 & 0.367 & 0.374 \\
 Adjusted $R^2$ & 0.235 & 0.257 & 0.162 & 0.198 & 0.278 & 0.326 & 0.319 \\
 Residual Std. Error & 4.548(df = 46) & 17.943(df = 46) & 17.649(df = 47) & 19.652(df = 46) & 18.078(df = 48) & 17.583(df = 46) & 15.810(df = 45)  \\
 F Statistic & 6.031$^{***}$ & 6.646$^{***}$ & 5.726$^{***}$ & 5.027$^{***}$ & 19.872$^{***}$ & 8.899$^{***}$ & 6.732$^{***}$ \\
 & (df = 3.0; 46.0) & (df = 3.0; 46.0) & (df = 2.0; 47.0) & (df = 3.0; 46.0) & (df = 1.0; 48.0) & (df = 3.0; 46.0) & (df = 4.0; 45.0) \\
\hline
\hline \\[-1.8ex]
\textit{Note:} & \multicolumn{7}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}
\caption{Predicting sustainability scores from the socio-economic indicators of states.}
\label{6goals_no_interactions}
\end{table}

\end{comment}
